Delay-Constrained Topology-Transparent Distributed Scheduling for MANETs

Transparent topology is common in many mobile ad hoc networks (MANETs) such as vehicle ad hoc networks (VANETs), unmanned aerial vehicle (UAV) ad hoc networks, and wireless sensor networks due to their decentralization and mobility nature. There are many existing works on distributed scheduling scheme design for topology-transparent MANETs. Most of them focus on delay-unconstrained settings. However, with the proliferation of real-time applications over wireless communications, it becomes more and more important to support delay-constrained traffic in MANETs. In such applications, each packet has a given hard deadline: if it is not delivered before its deadline, its validity will expire and it will be removed from the system. This feature is fundamentally different from the traditional delay-unconstrained one. In this paper, we for the first time investigate distributed scheduling schemes for a topology-transparent MANET to support delay-constrained traffic. We analyze and compare probabilistic ALOHA scheme and deterministic sequence schemes, including the conventional time division multiple access (TDMA), the Galois field (GF) sequence scheme proposed in \cite{chlamtac1994making}, and the combination sequence scheme that we propose for a special type of sparse network topology.We use both theoretical analysis and empirical simulations to compare all these schemes and summarize the conditions under which different individual schemes perform best.

==> reuse.tex <==
\section{GPS-Enabled Frequency/Sequence Reuse} \label{sec:reuse}
According to our interference model, if the distance of two
transmitters are larger than $2R$, they are not interferer of each other and thus can
transmit simultaneously (or equivalently share the same sequence).
This idea is same as spectrum reuse in cellular networks \cite{mac1979advanced}.
However, in our current topology-transparent setting, it is impossible to know which two transmitters
have distance larger than $2R$.
Thus, in our current sequence design in Sec.~\ref{sec:sequence},
a sequence cannot be allocated to more than one user to avoid collision.

To exploit the benefit of spectrum reuse, Wong in \cite{wong2014transmission} proposed a
Global Positioning System (GPS)-enabled sequence reuse scheme to improve the system performance.
The solution can also be directly applied to our problem  to further improve the system average timely throughput.
We will first briefly introduce the GPS-enabled sequence reuse scheme and then show our GPS-enabled TDMA and GF schemes.

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=\linewidth]{fig/cellular}\\
  \caption{Cellular network.}\label{fig:cellular}
\end{figure}

We assume that all transmitters are distributed in a 2-D plane
and the distance between any two transmitters is larger than or equal to $d_{\min}$.


We divide the plane by using regular hexagonal tiling cells with cell radius $h = \frac{d_{\min}}{\sqrt{3}}$
as shown in Fig.~\ref{fig:cellular}. We can further consider a planar coordinate
system with the axes intersecting at a $60^{\circ}$ angle instead of
orthogonally. We can define a regular tiling of the plane by
hexagonal cells with centers $(md_{\min}, nd_{\min})$
for all integers $m$ and $n$. We further assume that any transmitter
is located at the center of a hexagonal cell in Fig.~\ref{fig:cellular}.
To exploit the benefit of spectrum reuse, we only need to
guarantee any two users whose distance is within $2R$
do not share the same sequence. In another words, we need to find
a set of distinct sequences to cover all cells in the plane such that
any two transmitters whose distance is within $2R$ do not share the same sequence.
Let $G$ be the smallest integer satisfying
\be
G = b_1^2 + b_1b_2 + b_2^2 \ge \left(\frac{2R}{d_{\min}} \right)^2
\ee
where $b_1$ and $b_2$ are two nonnegative integers.
Wong in \cite{wong2014transmission} proved that there exists an allocation
scheme to cover the whole plane by using $G$ distinct sequences.

For GPS-enabled TDMA, the sequence period is $G$ instead of $N$.
For GPS-enabled GF-based code, we need to find a prime power $q$ and an integer $k$ such that
\bee
q-kD \ge 1 \nnb \\
q^{k+1} \ge G, \nnb
\eee
which is exactly $q(D,G)$ and the corresponding sequence period is $L=q^2(D,G)$.


\begin{figure}[t]
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=\linewidth]{fig/period_comparision_N=2000_D=4_G=421}\\
  \caption{Sequence period of conventional TDMA/GF and GPS-enabled TDMA/GF. \label{fig:reuse_compare}}
\end{figure}


As shown in Lemma~\ref{lem:R-1-R-2-decrease-with-L}, the sequence period
is one main performance indicator. In terms of the lower bound of system timely throughput,
the less the sequence period, the better the system performance.
We then compare the sequence period of conventional TDMA sequence, conventional GF-based sequence,
GPS-enabled TDMA sequence, and GPS-enabled GF-based sequence with respect to different number of pairs, i.e., $N$,
We can consider a specific setting: e.g., $d_{\min}=10, R=100, D=2$. In this case, we can find that $G=421$ and $q(D,G)=9$.
The results are shown in Fig.~\ref{fig:reuse_compare}. We can see that when is small, the conventional TDMA/GF approaches are better
than the GPS-enabled ones. But when $N$ is larger enough, the GPS-based ones becomes better and in principle they can
support infinite number of pairs in the plane.






